Annotations as Rollouts: Efficient and Scalable Reinforcement Learning for Video MLLMs

Multimodal large language models (MLLMs) have become a prevailing paradigm for unified video perception. However, post-training on large multi-task datasets remains challenging, as existing reinforcement learning methods sample on-policy groups with few high-quality rollouts even with costly chain-of-thought (CoT) generation. In this paper, we study the sample efficiency and scalability of RL post-training for video MLLMs and introduce OraRL. We identify an overlooked role for annotations: Beyond scoring rollouts, each can enter its on-policy group as an oracle rollout, a direct positive optimization target. Direct oracle integration, however, is nontrivial: a high-reward oracle raises the group baseline and inverts otherwise positive policy advantages, a failure we term advantage inversion. At the core of OraRL is a decoupled advantage estimator: policy rollouts determine an oracle-free baseline, while the oracle-policy gap modulates both a directional gain and a separate detached oracle advantage. Sign-balanced pruning improves efficiency: by retaining only the oracle and the strongest rollouts of each sign, OraRL requires just 2.2x the step time of SFT, less than half the 4.9x required by GRPO with CoT. OraRL scales with model size and data, surpassing its backbone from 0.8B to 9B and GRPO up to 100k prompts. Without chain-of-thought, Video-ORA-9B decodes in 130 ms instead of 4,780 ms. Compared with the respective prior best models, it raises temporal mIoU from 62.5 to 66.0, tracking AO from 73.0 to 78.2, segmentation from 64.3 to 70.4, and the three-benchmark spatial-intelligence macro average from 51.0 to 56.1; on VSI-Bench, it scores 73.1 against 55.0 for GPT-5 and 55.1 for Gemini-3-Pro.

==> figs/task_demo_common_tikz.tex <==
% Shared styles and geometry for the full-width qualitative demo pages.
% Input inside a local group before each task-specific tikzpicture.
%
% Card layout, top to bottom: example label, prompt, frame strip, and two
% full-width output bands (GT above, PRED below). Colour language: amber and
% dashed marks the annotation, the paper's green and solid marks \modelname{}
% output, and slate is reserved for neutral chrome.

\definecolor{qdink}{HTML}{20252A}
\definecolor{qdmuted}{HTML}{697078}
\definecolor{qdslate}{HTML}{46586B}
\definecolor{qdrule}{HTML}{D2D8DE}
\definecolor{qdgtc}{HTML}{B57A18}
\definecolor{qdgtfillc}{HTML}{FBF3E4}
\definecolor{qdgtlinec}{HTML}{E0C48F}
\definecolor{qdprc}{HTML}{2F6E5C}
\definecolor{qdprfillc}{HTML}{EAF2EF}
\definecolor{qdprlinec}{HTML}{8FB4A9}

\def\qdPageW{18.00}
\def\qdPageH{22.70}
\def\qdCardX{0.25}
\def\qdCardW{17.50}
\def\qdCardH{6.72}
\def\qdRowOne{14.23}
\def\qdRowTwo{7.19}
\def\qdRowThree{0.15}
\def\qdTextL{0.70}
\def\qdTextR{17.30}
\def\qdTagX{0.98}
\def\qdBandTextX{2.05}

\tikzset{
  qdcard/.style={
    rounded corners=2.4pt,
    draw=qdrule,
    line width=0.45pt,
    fill=white
  },
  qdframe/.style={
    rounded corners=1.4pt,
    draw=qdrule,
    line width=0.5pt
  },
  qdgtfill/.style={
    rounded corners=2.2pt,
    draw=qdgtlinec,
    line width=0.5pt,
    fill=qdgtfillc
  },
  qdprfill/.style={
    rounded corners=2.2pt,
    draw=qdprlinec,
    line width=0.5pt,
    fill=qdprfillc
  },
  qdexample/.style={
    font=\footnotesize\bfseries,
    text=qdslate,
    inner sep=0pt
  },
  qdnote/.style={
    font=\footnotesize,
    text=qdmuted,
    inner sep=0pt
  },
  qdbody/.style={
    font=\small,
    text=qdink,
    inner sep=0pt,
    align=left
  }
}

\newcommand{\qdcode}[1]{{\ttfamily\detokenize{#1}}}

% #1 task title, #2 family tag, #3 subtitle, #4 interface summary.
\newcommand{\qdheader}[4]{%
  \node[anchor=west,font=\Large\bfseries,text=qdink,inner sep=0pt]
    at (0.35,22.40) {#1};
  \node[anchor=east,font=\footnotesize\bfseries,text=qdslate,inner sep=0pt]
    at (17.65,22.40) {#2 \enspace$\cdot$\enspace 3 EXAMPLES};
  \node[anchor=west,font=\small,text=qdmuted,inner sep=0pt]
    at (0.35,21.78) {#3};
  \node[anchor=east,font=\footnotesize,text=qdslate,inner sep=0pt]
    at (17.65,21.78) {#4};
  \draw[qdslate,line width=0.8pt] (0.35,21.32) -- (17.65,21.32);
}

% #1 row bottom, #2 example number, #3 category, #4 right-aligned outcome note.
\newcommand{\qdcardbase}[4]{%
  \draw[qdcard]
    (\qdCardX,#1)
    rectangle ({\qdCardX+\qdCardW},{#1+\qdCardH});
  \fill[qdslate,rounded corners=0.9pt]
    (\qdCardX,#1)
    rectangle ({\qdCardX+0.14},{#1+\qdCardH});
  \node[qdexample,anchor=west] at (\qdTextL,{#1+6.44})
    {EXAMPLE #2 \enspace$\cdot$\enspace #3};
  \node[qdnote,anchor=east] at (\qdTextR,{#1+6.44}) {#4};
}

% #1 row bottom, #2 prompt body.
\newcommand{\qdprompt}[2]{%
  \node[qdbody,anchor=north west,text width=16.60cm]
    at (\qdTextL,{#1+6.11}) {#2};
}

% Annotation band. #1 row bottom, #2 band bottom, #3 band top, #4 payload.
\newcommand{\qdgtband}[4]{%
  \draw[qdgtfill]
    (\qdTextL,{#1+#2})
    rectangle (\qdTextR,{#1+#3});
  \node[anchor=north west,font=\footnotesize\bfseries,text=qdgtc,inner sep=0pt]
    at (\qdTagX,{#1+#3-0.20}) {GT};
  \node[
    anchor=north west,
    font=\footnotesize\ttfamily,
    text=qdink,
    inner sep=0pt,
    align=left
  ] at (\qdBandTextX,{#1+#3-0.20}) {#4};
}

% Model prediction band, geometrically identical to \qdgtband.
\newcommand{\qdpredband}[4]{%
  \draw[qdprfill]
    (\qdTextL,{#1+#2})
    rectangle (\qdTextR,{#1+#3});
  \node[anchor=north west,font=\footnotesize\bfseries,text=qdprc,inner sep=0pt]
    at (\qdTagX,{#1+#3-0.20}) {PRED};
  \node[
    anchor=north west,
    font=\footnotesize\ttfamily,
    text=qdink,
    inner sep=0pt,
    align=left
  ] at (\qdBandTextX,{#1+#3-0.20}) {#4};
}

% Frame shown at its native aspect ratio, so that normalized overlay
% coordinates map linearly onto the drawn rectangle.
% #1 file, #2 x, #3 y bottom, #4 width, #5 height, #6 label.
\newcommand{\qdframe}[6]{%
  \begin{scope}
    \clip[rounded corners=1.4pt]
      (#2,#3) rectangle ({#2+#4},{#3+#5});
    \node[inner sep=0pt]
      at ({#2+0.5*#4},{#3+0.5*#5})
      {\includegraphics[height=#5cm]{#1}};
  \end{scope}
  \draw[qdframe] (#2,#3) rectangle ({#2+#4},{#3+#5});
  \node[
    anchor=north west,
    rounded corners=1.0pt,
    fill=white,
    fill opacity=0.90,
    text opacity=1,
    inner xsep=2.0pt,
    inner ysep=1.2pt,
    font=\footnotesize\bfseries,
    text=qdslate
  ] at ({#2+0.10},{#3+#5-0.10}) {#6};
}

% Same frame with the label moved to the bottom-left corner, for panels whose
% upper region is occupied by overlays.
\newcommand{\qdframelow}[6]{%
  \begin{scope}
    \clip[rounded corners=1.4pt]
      (#2,#3) rectangle ({#2+#4},{#3+#5});
    \node[inner sep=0pt]
      at ({#2+0.5*#4},{#3+0.5*#5})
      {\includegraphics[height=#5cm]{#1}};
  \end{scope}
  \draw[qdframe] (#2,#3) rectangle ({#2+#4},{#3+#5});
  \node[
    anchor=south west,
    rounded corners=1.0pt,
    fill=white,
    fill opacity=0.90,
    text opacity=1,
    inner xsep=2.0pt,
    inner ysep=1.2pt,
    font=\footnotesize\bfseries,
    text=qdslate
  ] at ({#2+0.10},{#3+0.10}) {#6};
}

% Box overlays. Coordinates are normalized to 0--1000 with y pointing down.
% The annotation is always drawn last so that, where the two boxes coincide,
% the prediction stays visible through the gaps of the dashed outline. Its
% casing therefore follows the same dash pattern.
% #1 frame x, #2 frame y bottom, #3 frame width, #4 frame height,
% #5 x0, #6 y0, #7 x1, #8 y1.
\newcommand{\qdgtrect}[8]{%
  \draw[white,line width=2.1pt,opacity=0.75,dash pattern=on 2.2pt off 1.5pt]
    ({#1+#3*(#5)/1000},{#2+#4*(1000-(#6))/1000})
    rectangle ({#1+#3*(#7)/1000},{#2+#4*(1000-(#8))/1000});
  \draw[qdgtc,line width=1.0pt,dash pattern=on 2.2pt off 1.5pt]
    ({#1+#3*(#5)/1000},{#2+#4*(1000-(#6))/1000})
    rectangle ({#1+#3*(#7)/1000},{#2+#4*(1000-(#8))/1000});
}

\newcommand{\qdpredrect}[8]{%
  \draw[white,line width=2.1pt,opacity=0.65]
    ({#1+#3*(#5)/1000},{#2+#4*(1000-(#6))/1000})
    rectangle ({#1+#3*(#7)/1000},{#2+#4*(1000-(#8))/1000});
  \draw[qdprc,line width=1.0pt]
    ({#1+#3*(#5)/1000},{#2+#4*(1000-(#6))/1000})
    rectangle ({#1+#3*(#7)/1000},{#2+#4*(1000-(#8))/1000});
}

% Predicted point prompts. #1..#4 frame geometry, #5 x, #6 y.
\newcommand{\qdpospoint}[6]{%
  \fill[white,opacity=0.85]
    ({#1+#3*(#5)/1000},{#2+#4*(1000-(#6))/1000}) circle (0.085);
  \fill[qdprc]
    ({#1+#3*(#5)/1000},{#2+#4*(1000-(#6))/1000}) circle (0.055);
}

\newcommand{\qdnegpoint}[6]{%
  \fill[white,opacity=0.85]
    ({#1+#3*(#5)/1000},{#2+#4*(1000-(#6))/1000}) circle (0.085);
  \draw[qdprc,line width=0.7pt]
    ({#1+#3*(#5)/1000-0.055},{#2+#4*(1000-(#6))/1000-0.055})
    -- ({#1+#3*(#5)/1000+0.055},{#2+#4*(1000-(#6))/1000+0.055});
  \draw[qdprc,line width=0.7pt]
    ({#1+#3*(#5)/1000-0.055},{#2+#4*(1000-(#6))/1000+0.055})
    -- ({#1+#3*(#5)/1000+0.055},{#2+#4*(1000-(#6))/1000-0.055});
}

% Timeline carrying the annotated span above the axis and the predicted span
% below it. #1 row bottom, #2 axis offset, #3--#4 GT fractions,
% #5--#6 prediction fractions, #7 GT label, #8 prediction label, #9 duration.
\newcommand{\qdtimelinepair}[9]{%
  \draw[qdrule,line width=1.4pt,line cap=round]
    (2.40,{#1+#2}) -- (15.60,{#1+#2});
  \node[anchor=east,font=\footnotesize,text=qdmuted,inner sep=0pt]
    at (2.20,{#1+#2}) {0\,s};
  \node[anchor=west,font=\footnotesize,text=qdmuted,inner sep=0pt]
    at (15.80,{#1+#2}) {#9};
  \draw[qdgtc,line width=3.0pt,line cap=round]
    ({2.40+13.20*(#3)},{#1+#2+0.11}) -- ({2.40+13.20*(#4)},{#1+#2+0.11});
  \draw[qdprc,line width=3.0pt,line cap=round]
    ({2.40+13.20*(#5)},{#1+#2-0.11}) -- ({2.40+13.20*(#6)},{#1+#2-0.11});
  \node[anchor=south,font=\footnotesize\bfseries,text=qdgtc,inner sep=1.4pt]
    at ({2.40+13.20*((#3)+(#4))/2},{#1+#2+0.15}) {#7};
  \node[anchor=north,font=\footnotesize\bfseries,text=qdprc,inner sep=1.4pt]
    at ({2.40+13.20*((#5)+(#6))/2},{#1+#2-0.15}) {#8};
}

